A Simple Semantics and Static Analysis for Stack Inspection

The Java virtual machine and the .NET common language runtime feature an access control mechanism specified operationally in terms of run-time stack inspection. We give a denotational semantics in "eager" form, and show that it is equivalent to the "lazy" semantics using stack inspection. We give a static analysis of safety, i.e., the absence of security errors, that is simpler than previous proposals. We identify several program transformations that can be used to remove run-time checks. We give complete, detailed proofs for safety of the analysis and for the transformations, exploiting compositionality of the eager semantics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{284}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.17}{10.4204/EPTCS.129.17}}

